CO2 Forest: Improved Random Forest by Continuous Optimization of Oblique Splits

We propose a novel algorithm for optimizing multivariate linear threshold functions as split functions of decision trees to create improved Random Forest classifiers. Standard tree induction methods resort to sampling and exhaustive search to find good univariate split functions. In contrast, our method computes a linear combination of the features at each node, and optimizes the parameters of the linear combination (oblique) split functions by adopting a variant of latent variable SVM formulation. We develop a convex-concave upper bound on the classification loss for a one-level decision tree, and optimize the bound by stochastic gradient descent at each internal node of the tree. Forests of up to 1000 Continuously Optimized Oblique (CO2) decision trees are created, which significantly outperform Random Forest with univariate splits and previous techniques for constructing oblique trees. Experimental results are reported on multi-class classification benchmarks and on Labeled Faces in the Wild (LFW) dataset.

==> fig/datasets.tex <==
\begin{table}
  \begin{center}
    \begin{tabular}{|@{~}c@{~}|@{~}c@{~}@{~}c@{~}@{~}c@{~}@{~}c@{~}|}
      \hline
      Name      & Train     & Test     & Classes & Dim   \\
      \hline
      Connect4$^*$  & $55,000^*$  & $12,557^*$ & $3$ &$126$ \\
      Covertype$^*$ & $500,000^*$ & $81,012^*$ & $7$ & $54$ \\
      %% DNA       & $2,000$     & $1,186$    & $180$ & $3$ \\
      \hline
      Letter        & $15,000$    & $5,000$    & $26$ & $16$  \\
      MNIST         & $60,000$    & $10,000$   & $10$ & $784$ \\
      \hline
      Pendigits     & $7,494$     & $3,498$    & $10$ & $16$  \\
      Protein       & $17,766$    & $6,621$    & $3$  & $357$ \\
      \hline
     SatImage      & $4,435$     & $2,000$    & $6$  & $36$  \\
      Segment$^*$   & $1,848^*$   & $462^*$    & $7$  & $19$  \\
      \hline
      USPS          & $7,291$     & $2,007$    & $10$ & $256$ \\
      SensIT        & $78,823$    & $19,705$   & $3$  &$100$  \\
      \hline
    \end{tabular}
  \end{center}
  \caption{ \label{tab:multi-class-data}
    Multi-class classification benchmarks and their number of
    training and test points, number of classes, and feature
    dimensionality.
  }
\end{table}


==> fig/forest_errors.tex <==
\begin{table*}
  %\small
  \begin{center}
    \begin{tabular}{|l|ccc||ccc||ccc|}
      \hline
      Dataset
      & \multicolumn{3}{@{\,}c@{\,}||}{Random Forest Err\,(\%)}
      & \multicolumn{3}{@{\,}c@{\,}||}{OC1 Forest Err\,(\%)}
      & \multicolumn{3}{@{\,}c@{\,}|}{CO2 Forest Err\,(\%)}\\
      & 10 & 30 & 1000 & 10 & 30 & 1000 & 10 & 30 & 1000\\
      \hline
      Connect4  & 18.9 & 17.4 & 16.2   &  &     &      &     17.1 & 15.7 & 14.7\\
      Covertype & 3.2 & 2.8 & 2.6    &   &     &      &    3.1 & 2.7 & 2.6\\
      \hline
      Letter    & 6.6 & 4.7 & 3.7    &  7.6 & 5.0 & 3.8  &   3.2 & 2.3 & 1.8\\
      MNIST     & 4.5 & 3.5 & 2.8    &      &     &      &   2.5 & 2.0 & 1.9\\
      \hline
      Pendigits & 3.9 & 3.3 & 3.5    &  3.2 & 2.2 & 2.3  &   1.8 & 1.7 & 1.7\\
      Protein   & 39.9 & 35.5 & 30.9 &      &     &      &  33.8 & 31.2 & 30.3\\
      \hline
      Satimage  & 10.1 & 9.4 & 8.9   &  10.1 & 9.85 & 9.5 &   9.6 & 9.1 & 8.9\\
      Segment   & 4.5 & 3.5 & 2.8    &      &     &       &   2.8 & 2.4 & 2.4\\
      \hline
      USPS      & 9.0 & 7.2 & 6.4    &      &     &      &   5.8 & 5.9 & 5.5\\
      SensIT    & 15.5 & 14.0 & 13.4 &      &     &      &   14.1 & 13.0 & 12.5\\
      \hline
    \end{tabular}
  \end{center}
  \caption{
    \label{tab:multi-class-results}
    Test error rates (\%) for Random Forest \vs~CO2 Forest with
    $10$, $30$, $1000$ trees on corresponding classification benchmarks
    from \tabref{tab:multi-class-data}.
  }
\end{table*}


==> fig/forest_errors2.tex <==
\begin{table*}
\renewcommand{\arraystretch}{1.3}
\begin{center}
\begin{tabular}{|c||cccc||ccc||ccc||ccc|}
\hline
  \multicolumn{5}{|c||}{}
& \multicolumn{9}{c|}{\bf Test error (\%) with different number of trees} \\
\cline{6-14}
\multicolumn{5}{|c||}{\bf Dataset Information}
& \multicolumn{3}{ c||}{\bf Random Forest}
& \multicolumn{3}{ c||}{\bf OC1 Forest}
& \multicolumn{3}{ c| }{\bf CO2 Forest}\\\cline{1-5}
\bf Name      & \bf \#Train     & \bf \#Test     & \bf \#Class & \bf Dim &
\bf 10 & \bf 30 & \bf 1000 & \bf 10 & \bf 30 & \bf 1000 & \bf 10 & \bf 30 &
\bf 1000\\
\hline
Segment$^*$   & $1,848$   & $462$    & $7$  & $19$  &
4.5 & 3.5 & 2.8   &   2.6 & 2.4 & 1.9 &   2.8 & 2.4 & 2.4 \\
SatImage      & $4,435$     & $2,000$    & $6$  & $36$  &
10.1 & 9.4 & 8.9   &  10.1 & 9.9 & 9.5 &   9.6 & 9.1 & 8.9 \\
\hline
USPS          & $7,291$     & $2,007$    & $10$ & $256$ &
9.0 & 7.2 & 6.4    &  7.1 &  7.1 & 6.8  &   5.8 & 5.9 & 5.5 \\
Pendigits     & $7,494$     & $3,498$    & $10$ & $16$  &
3.9 & 3.3 & 3.5    &  3.2 &  2.2 & 2.3  &   1.8 & 1.7 & 1.7 \\
\hline
Letter        & $15,000$    & $5,000$    & $26$ & $16$  &
6.6 &  4.7 &  3.7 &  7.6 &  5.0 & 3.8  &   3.2 & 2.3 & 1.8 \\
Protein       & $17,766$    & $6,621$    & $3$  & $357$ &
39.9 & 35.5 & 30.9 & 39.1 & 34.6 & 30.8 &  33.8 & 31.2 & 30.3 \\
\hline
Connect4$^*$  & $55,000$  & $12,557$ & $3$ &$126$ &
18.9 & 17.4 & 16.2 & %% 24.9** & 23.4** & 22.6**
\multicolumn{3}{c||}{\multirow{2}{*}{\change{N/A}}} & 17.1 & 15.7 & 14.7 \\
%% DNA       & $2,000$     & $1,186$    & $180$ & $3$ \\
MNIST         & $60,000$    & $10,000$   & $10$ & $784$ &
4.5 &  3.5 &  2.8 &    &     &      &   2.5 & 2.0 & 1.9
\\
\hline
SensIT        & $78,823$    & $19,705$   & $3$  &$100$ &
15.5 & 14.0 & 13.4 &  %% 19.2** & 17.8** & 17.1**
\multicolumn{3}{c||}{\multirow{2}{*}{\change{N/A}}} & 14.1 & 13.0 & 12.5 \\
Covertype$^*$ & $500,000$ & $81,012$ & $7$ & $54$ &
3.2 &  2.8 &  2.6 &  %% 25.6** & 24.0** & 23.2**
& & &    3.1 & 2.7 & 2.6 \\
\hline
\end{tabular}
\vspace*{.2cm}
\caption{Test error rates of different forests with different number
  of trees on multi-class classification benchmarks. Firs few columns
  provide dataset information including number of training and test
  points, number of classes, and feature dimensionality. Test error
  rates (\%) for Random Forest, OC1 Forest, and CO2 Forest with $10$,
  $30$, and $1000$ trees are reported. For datasets marked with a
  ``$^*$'' (\ie~Segment, Connect4, Covertype) we do not have access to
  prespecified test and training splits, hence we use our own
  splits. As the number of training data points increases, OC1 pecomes
  extremely slow, so this method is not applicable to the datasets
  with $50,000$ or more training data points.}
\end{center}
\label{tab:multi-class-data}
\label{tab:multi-class-results}
\end{table*}


==> fig/jaccards.tex <==
\begin{table}
\begin{center}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{|ccc|}
  \hline
  \textbf{Split Function} & \textbf{16 trees} & \textbf{32 trees} \\
  \hline
  Axis-aligned Forest        & 32.28 & 34.61 \\
  Two-feature probe Forest   & 36.03 & 38.61 \\
  CO2 Forest                 & 40.33 & 42.55 \\
  \hline
\end{tabular}
\end{center} 
\caption{ \label{tab:jaccards}
  Jaccard scores comparing CO2 Forest to baseline forest constructions on
  the Labeled Faces in the Wild (LFW) dataset.
}
\end{table}


==> fig/lfw_limits.tex <==
\begin{figure}
  \begin{center}
    \includegraphics[height = 0.38\linewidth]{tikz/lfw_height_pdf.pdf}
    \nolinebreak[4]
    \includegraphics[height = 0.38\linewidth]{tikz/lfw_trees_pdf.pdf}
  \end{center}
  \caption{Test Jaccard scores on LFW for
    (left) forests with different tree depth, (right) forests with
    different number of trees. On the left, we consider forests of
    $16$ trees with diffent limit on the tree depth from $10$ to
    $30$. The plot on the right shows the Jaccard score as a function
    of the number trees in the forest.}
  \label{fig:lfw_limits}
\end{figure}

